Multi-layer optimisation of hybrid energy storage systems for electric vehicles

This research presents a multi-layer optimization framework for hybrid energy storage systems (HESS) for passenger electric vehicles to increase the battery system's performance by combining multiple cell chemistries. Specifically, we devise a battery model capturing voltage dynamics, temperature and lifetime degradation solely using data from manufacturer datasheets, and jointly optimize the capacity distribution between the two batteries and the power split, for a given drive cycle and HESS topology. The results show that the lowest energy consumption is obtained with a hybrid solution consisting of a NCA-NMC combination, since this provides the best trade-off between efficiency and added weight.

==> Sections/7acknowledgements.tex <==
\section{Acknowledgement}
I want to express my gratitude towards my supervisors Dr. Ir. Theo Hofman and Ir. Jorn van Kampen for their guidance and input during this research. 
I would like to express my gratitude to my colleagues in the battery research group for their support and insightful discussions, which greatly helped me enhance the quality of this thesis.

==> Sections/comment.tex <==
\begin{comment}   

\begin{subequations}
\begin{align}
    &I_\mathrm{\{E,P\},{min}}\leq I_\mathrm{\{E,P\}}\leq I_\mathrm{\{E,P\},{max}}\\
    &V_\mathrm{\{E,P\},{Min}}\leq V_\mathrm{OCV,\{E,P\}}-I_\mathrm{\{E,P\}}\cdot R_\mathrm{\{E,P\}}\leq V_\mathrm{\{E,P\},{Max}}
    \\
    &P_{\mathrm{M}}-\eta_\mathrm{DC}\cdot I_\mathrm{E}(V_\mathrm{E,OCV}-I_\mathrm{E}\cdot R_\mathrm{E})-I_\mathrm{P}(V_\mathrm{P,OCV}-I_\mathrm{P}\cdot R_\mathrm{P})=0
\end{align}
\end{subequations}

\hl{vanaf hier commenten}


\end{comment}

\begin{comment}
\section{PMP problem definition}
States are $SoC(t)$ of both batteries with
\begin{subequations}
    \begin{align}
        x(t)=\begin{bmatrix}
             SoC_\mathrm{E}(t)\\
             SoC_\mathrm{P}(t)
        \end{bmatrix}
        =\begin{bmatrix}
             \int_{0}^{t}I_\mathrm{E}(t)/\mathcal{Q}_E\; dt\\
             \int_{0}^{t}I_\mathrm{P}(t)/\mathcal{Q}_P\; dt
             \end{bmatrix}
    \end{align}
\end{subequations}
Therefore the system dynamics are
\begin{subequations}
    \begin{align}
        \dot{x}(t)=\begin{bmatrix}
             I_\mathrm{E}(t)/\mathcal{Q}_E \\
             I_\mathrm{P}(t)/\mathcal{Q}_P 
             \end{bmatrix}
    \end{align}
\end{subequations}
control parameter $u(t)=P_\mathrm{DC}(t)$
    \begin{align} 
        {u}(t)=P_\mathrm{DC}(t)=\eta_\mathrm{DC}\cdot(V_\mathrm{OC}(x_\mathrm{1})\cdot I_\mathrm{E}(t)-R_\mathrm{E}(x_1)\cdot I_\mathrm{E}^2(t))
    \end{align}
    for the second power $P_\mathrm{P}(t)$ can be rewritten to
    \begin{equation}
\begin{split}
         P_\mathrm{P}(t)=V_\mathrm{OC}(x_\mathrm{2})\cdot I_\mathrm{E}(t)-R_\mathrm{P}(x_2)\cdot I_\mathrm{E}^2(t)\\=P_\mathrm{M}(t)-P_\mathrm{DC}(t)=P_\mathrm{M}(t)-u(t)
\end{split}
\end{equation}
Combining \cref{eq:xdot1} with \cref{eq:P_Dctocurrent} and \cref{eq:P_powertocurrent} leads to.
\begin{align}
    \begin{split}   
    \renewcommand{\arraystretch}{3}
        \dot{x}(t)=\begin{bmatrix}
            \frac{V_\mathrm{OC,E}(x_\mathrm{1})-\sqrt{V_\mathrm{OC,E}(x_\mathrm{1})^2-4\cdot u(t)\cdot\eta_\mathrm{DC}^{-1}\cdot R_\mathrm{E}(x_\mathrm{1})}}{\mathcal{Q}_\mathrm{E}\cdot2\cdot R_\mathrm{E}(x_1)}\\
            \frac{V_\mathrm{OC,P}(x_\mathrm{2})-\sqrt{V_\mathrm{OC,P}(x_\mathrm{2})^2-4\cdot(P_\mathrm{M}(t)-u(t))\cdot R_\mathrm{P}(x_\mathrm{2})}}{\mathcal{Q}_\mathrm{P}\cdot2\cdot R_\mathrm{E}(x_1)}
             \end{bmatrix}
    \end{split}
\end{align}
We can rewrite \cref{eq:xdot2} to 

\begin{align}
    \begin{split}   
    \renewcommand{\arraystretch}{1.5}
        \dot{x}(t)=\begin{bmatrix}
f_\mathrm{1}(x_\mathrm{1},u(t))\\f_\mathrm{2}(x_\mathrm{2},u(t),P_\mathrm{M}(t))        
             \end{bmatrix}
    \end{split}
\end{align}
Since we can rewrite the system constraints \labelcref{eq:optimisationconstraints} as constraints on the control variable $u(t)=P_\mathrm{DC}$, we can solve the control problem unconstrained under the condition that $u(t)\in \mathcal{U}$ where $\mathcal{U}$ is the searchgrid adhering to constraints defined in \cref{eq:PDCconstraints}.
\par \noindent
\Cref{eq:Unconstrainedham} describes the resulting unconstrained Hamiltonian for the system. 
\begin{align}\label{eq:Unconstrainedham}
\begin{split}
    H=\lambda_\mathrm{1}(t)\cdot f_\mathrm{1}(x_\mathrm{1},u(t),t)+\lambda_\mathrm{2}(t)\cdot f_\mathrm{2}(x_\mathrm{2},u(t),P_\mathrm{M}(t))\\+
    L(x_\mathrm{1}(t),x_\mathrm{2}(t),u(t),t) 
\end{split}
\end{align}
Where $L(x_\mathrm{1}(t),x_\mathrm{2}(t),u(t),t)$ is the instantaneous cost $\dot{J}_\mathrm{TCO}$\labelcref{eq:TCOinstant}
the optimal control policy $u^*(t)$ can be determined by computing the argument at which the Hamiltonian is minimal on every time instance of the cycle.
We can only define a value for the Hamiltonian if we know the value for the costate at that instance. The Costate dynamics are defined by the partial derivative of the Hamiltonian to the states.
\begin{align}
    \dot{\lambda}(t)=\left. -\pdv{ H}{ x}\right|_{u_\mathrm{t}}
\end{align}



\begin{align}\label{eq:costatedyn}
\renewcommand{\arraystretch}{1.5}
    \dot{\lambda}(t)=\begin{bmatrix}
\pdv{(f_\mathrm{1}(x_\mathrm{1},u(t),t)+L(x_\mathrm{1}(t),x_\mathrm{2}(t),u(t),t))}{x_\mathrm{1}}\\\pdv{(f_\mathrm{2}(x_\mathrm{2},u(t),P_\mathrm{M}(t))+L(x_\mathrm{1}(t),x_\mathrm{2}(t),u(t),t))}{x_\mathrm{2}}        
             \end{bmatrix}
\end{align}
The equations that define the cost function and system dynamics \labelcref{eq:capdegdisdyn,eq:TCOinstant,eq:xdot2} are all dependant on the systems states $x(t)$ through the $SoC$ dependency on the $V_\mathrm{oc}(SoC)$ and $R(SoC)$. Onori et al.\cite{Onori2016} reason that the influence of the $SoC$ on both  $V_\mathrm{oc}(SoC)$ and $R(SoC)$ are small during the drivecycle, we can ignore the influence. We rewrite \cref{eq:costatedyn} with the aforementioned assumption to \cref{eq:costatedynzero}. 
\begin{align}\label{eq:costatedynzero}
\renewcommand{\arraystretch}{1}
    \dot{\lambda}(t)\approx \begin{bmatrix}
0\\0        
             \end{bmatrix}
\end{align}

This means that the costates stay constant and are defined by the initial condition of the costates.

estimating optimal costates

\begin{align}
    \pdv{ H(u(t),\lambda)}{ u(t)}=0 
\end{align}

\begin{align}
    \pdv{ f(x(t),u(t),t)}{ u(t)}=\begin{bmatrix}
                 \frac{\eta_\mathrm{DC}^{-1}}{\mathcal{Q}_\mathrm{E}\cdot\sqrt{V_\mathrm{OC,E}^2-4*\eta_\mathrm{DC}^{-1}*u(t)*R_\mathrm{E}}}\\
            \frac{V_\mathrm{OC,P}(x_\mathrm{2})-\sqrt{V_\mathrm{OC,P}(x_\mathrm{2})^2-4\cdot(P_\mathrm{M}(t)-u(t))\cdot R_\mathrm{P}(x_\mathrm{2})}}{\mathcal{Q}_\mathrm{P}\cdot2\cdot R_\mathrm{E}(x_1)}
             \end{bmatrix}
\end{align}

\begin{subequations}
    \begin{align}
    \mathcal{P}_{\{E,P\},\mathrm{tot}}&= \frac{\mathcal{E}_{\mathrm{design}}}{\mathcal{S}_{\{E,P\}}\cdot V_{c,\{E,P\},\mathrm{nom}}\cdot\mathcal{Q}_{c,\{E,P\}}}\\ 
    &\Downarrow\nonumber\\
    \mathcal{P}_{P}&=\lceil\lambda\cdot\mathcal{P}_{P,\mathrm{tot}}\rceil\\
    \mathcal{P}_{E}&=\lceil(1-\lambda)\cdot\mathcal{P}_{E,\mathrm{tot}}\rceil
    \end{align}
\end{subequations}
\begin{subequations}
\begin{align}
    \frac{\mathcal{S}_{P}\cdot V_{c,\mathrm{nom}}\cdot\mathcal{Q}_\mathrm{P}}{\mathcal{E}_\mathrm{design}}<\lambda<1-\frac{\mathcal{S}_{E}\cdot V_{c,\mathrm{nom}}\cdot\mathcal{Q}_\mathrm{E}}{\mathcal{E}_\mathrm{design}}\\
    \lambda\geq\frac{ I_\mathrm{design}- \eta_{\mathrm{DCDC}}\cdot I_{c,E,\mathrm{max}}\cdot\mathcal{P}_{E,\mathrm{tot}}}{I_{c,P,\mathrm{max}}\cdot\mathcal{P}_{P,\mathrm{tot}}-\eta_{\mathrm{DCDC}}\cdot I_{c,E,\mathrm{max}}\cdot\mathcal{P}_{E,\mathrm{tot}}}
\end{align}
\end{subequations}
\end{comment}

==> Sections/costfigure.tex <==
\begin{figure*}[t]
\centering
\begin{subfigure}[b]{0.32\textwidth}
  \includegraphics[width=\linewidth]{Figures/costfigvtc4m35a.eps}
  \caption{NCA-NMC cost breakdown}
  \label{fig:resultnmc}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
  \includegraphics[width=\linewidth]{Figures/costfigLFPm35a.eps}
  \caption{NCA-LFP cost breakdown}
  \label{fig:resultsLFP}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
  \includegraphics[width=\linewidth]{Figures/costfigLTOm35a.eps}
  \caption{NCA-LTO cost breakdown}
  \label{fig:resultsLTO}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
  \includegraphics[width=\linewidth]{Figures/costfigvtc4m35aSOC.eps}
  \caption{NCA-NMC $\Delta SoC$}
  \label{fig:SOCcostNMC}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
  \includegraphics[width=\linewidth]{Figures/costfigLFPm35aSOC.eps}
  \caption{NCA-LFP $\Delta SoC$}
  \label{fig:SOCcostLFP}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
  \includegraphics[width=\linewidth]{Figures/costfigLTOm35aSOC.eps}
  \caption{NCA-LTO $\Delta SoC$}
  \label{fig:SOCcostLTO}
  \end{subfigure}
  \caption{Cost breakdown and $\Delta SoC$ for all combinations for different capacity distributions between the high-power battery and the high-energy battery. The bar in \cref{fig:resultnmc,fig:resultsLFP,fig:resultsLTO} represents the cost for a single cell battery constructed of only the power battery cell.}
\label{fig:costresults}
\end{figure*}
